Provably Efficient Reinforcement Learning in Decentralized General-Sum Markov Games

This paper addresses the problem of learning an equilibrium efficiently in general-sum Markov games through decentralized multi-agent reinforcement learning. Given the fundamental difficulty of calculating a Nash equilibrium (NE), we instead aim at finding a coarse correlated equilibrium (CCE), a solution concept that generalizes NE by allowing possible correlations among the agents' strategies. We propose an algorithm in which each agent independently runs optimistic V-learning (a variant of Q-learning) to efficiently explore the unknown environment, while using a stabilized online mirror descent (OMD) subroutine for policy updates. We show that the agents can find an $\epsilon$-approximate CCE in at most $\widetilde{O}( H^6S A /\epsilon^2)$ episodes, where $S$ is the number of states, $A$ is the size of the largest individual action space, and $H$ is the length of an episode. This appears to be the first sample complexity result for learning in generic general-sum Markov games. Our results rely on a novel investigation of an anytime high-probability regret bound for OMD with a dynamic learning rate and weighted regret, which would be of independent interest. One key feature of our algorithm is that it is fully \emph{decentralized}, in the sense that each agent has access to only its local information, and is completely oblivious to the presence of others. This way, our algorithm can readily scale up to an arbitrary number of agents, without suffering from the exponential dependence on the number of agents.

==> 3_bandit.tex <==

\section{Warm-Up: The Bandit Case}\label{sec:bandit}

As a warm-up, we start with the simple stochastic bandit case, where two players repeatedly interact in a single-stage team \citep{claus1998dynamics}. 
This is essentially a Markov team with a single state and $H=1$. 
A two-player finite single-stage team can be described by a tuple $(\mc{A},\mc{B}, \rho)$, where $\mc{A}$ and $\mc{B}$ are the finite \emph{action} spaces (or \emph{pure strategy} spaces) for player $1$ and player $2$, respectively, and $\rho=(P_{a,b}:a\in\mc{A},b\in\mc{B})$ is a collection of reward distributions with support $[0,1]$. The players interact for $T$ rounds. At each round $t$, player 1 chooses an action $a_t\in\mc{A}$, and simultaneously, player 2 chooses an action $b_t\in\mc{B}$. Both players receive the same reward $R_t$ drawn i.i.d from the reward distribution $P_{a_t,b_t}$. Slightly abusing the notation, we also use $R_t(a, b)$ to denote the random reward received at round $t$ to emphasize its dependence on the action pair $(a,b)$. We let $r:\mc{A}\times\mc{B}\ra [0,1]$ be the expected value of the reward function, i.e., $r(a,b) = \int_0^1 x dP_{a,b}(x)$. 


A player can randomize its actions when necessary. We use $\mu \in \Delta(\mc{A})$ and $\nu\in\Delta(\mc{B})$ to denote the \emph{mixed strategies} (or simply strategies) for player 1 and player 2, respectively. Given a mixed strategy pair $(\mu,\nu)$, the corresponding expected reward for the players is denoted by $\mb{E}_{\mu\times\nu}[r(a,b)]$, where $a\sim \mu$ and $b\sim \nu$. The objective of the players is to maximize the team cumulative reward. Let $\mu_t$ and $\nu_t$ be the mixed strategies chosen by the two players at round $t$. Define $\mu^\star$ to be the best fixed strategy in hindsight for player 1 with respect to the strategy trajectory of player 2, i.e., $\mu^\star \defeq \arg\max_{\mu \in \Delta(\mc{A})}\sum_{t=1}^T \ee_{\mu\times \nu_t}[r(a,b)]$. We use the notion of \emph{regret} to measure the sub-optimality of player 1's strategy with respect to $\mu^\star$:
\[
\text{Reg}(\mu^\star, T) \defeq \sum_{t=1}^T \left(\mb{E}_{\mu^\star \times\nu_t}[r(a,b)] -\mb{E}_{\mu_t\times\nu_t}[r(a,b)]\right).
\]
Define $\nu^\star$ and the corresponding regret $\text{Reg}(\nu^\star, T)$ for player 2 analogously. We again emphasize that in a decentralized paradigm, the two players are not allowed to observe the actions of each other. Otherwise, the players can always ``orchestrate'' their actions in a pre-programmed way that trivially solves the problem as a centralized one. In our decentralized setting, the players need to coordinate their exploration of the joint action space silently. In the following, we first show that each player can run a simple no-regret learning algorithm Exp3~\citep{auer2002nonstochastic} to achieve a sublinear regret with respect to its best fixed strategy in hindsight. Exp3 is a standard adversarial bandit algorithm, and for completeness we include the pseudo-code in Appendix~\ref{app:exp3}. 

\begin{lemma}\label{lemma:exp3}
	If player 1 runs the Exp3 algorithm, for any $p\in (0,1]$ and for any strategy trajectory of player 2, with probability at least $1-p$, its regret is upper bounded by $\text{Reg}(\mu^\star, T) = \widetilde{O}(\sqrt{A T})$. 
\end{lemma}

A similar result holds for player 2, i.e., $\text{Reg}(\nu^\star, T) = \widetilde{O}(\sqrt{B T})$. So far we have shown that each agent achieves a reward \emph{value} that converges to its best fixed response in hindsight, but we are more interested in extracting a \emph{strategy pair} from the learning process that constitutes an approximate Nash equilibrium. The following result states that the two players can find a Nash equilibrium with high probability by uniformly sampling a strategy pair from their strategy trajectories. 


\begin{theorem}\label{thm:exp3}
	Let the players run Exp3 for $T$ rounds, and let $\{\mu_t\}_{t=1}^T$ and $\{\nu_t\}_{t=1}^T$ be the resultant strategy trajectories of players 1 and 2, respectively. Let the two players uniformly draw a time index $t^\star$ from the set $[T]$ using a common random seed. For any $p \in (0,1]$, if $T = \widetilde{\Omega}(\max\{A,B\}/\epsilon^2)$, then $(\mu_{t^\star},\nu_{t^\star})$ is an $\epsilon$-approximate NE with probability at least $1-p$. 
\end{theorem}

\begin{remark}
	The assumption of a common source of randomness, also termed a correlation device, is standard in decentralized learning \citep{bernstein2009policy,arabneydi2015reinforcement,zhang2019online}. Note that the correlation device is never used to \emph{coordinate} the exploration and learning, but is simply used to synchronize the selection of the policies already generated. A common random seed is generally considered as a mild assumption  and does not break the decentralized paradigm. 
\end{remark}


It can be seen from the proof of Theorem~\ref{thm:exp3} that any no-regret learning algorithm against an adversarial reward sequence can achieve a similar result as in Theorem~\ref{thm:exp3}, and Exp3 is just a representative example of them. Interestingly, the usage of Exp3 is reminiscent of the empirical solution to address decentralized coordination in \citet{claus1998dynamics} for single-stage teams, where an independent learning algorithm with Boltzmann exploration was proposed. Our results can thus be viewed as a quantitative and non-asymptotic justification of this conceptual method. On the other hand, no-regret learning has been empirically shown to converge to Nash equilibria in coordination games \citep[Sec. 4.1]{jafari2001no}, but to the best of our knowledge, no theoretical justification has been provided.   

Exp3 seems conservative in presuming that the reward sequence is changing adversarially, while in fact the other agent is also updating its policy to maximize the same reward. In this sense, no-regret learning does not proactively foster cooperation, but only passively defends against the unobserved behavior of the teammate. This could be the reason why team-optimality is not guaranteed with no-regret learning, but only NE is. 


